Cooperative UAVs Gas Monitoring using Distributed Consensus

This paper addresses the problem of target detection and localisation in a limited area using multiple coordinated agents. The swarm of Unmanned Aerial Vehicles (UAVs) determines the position of the dispersion of stack effluents to a gas plume in a certain production area as fast as possible, that makes the problem challenging to model and solve, because of the time variability of the target. Three different exploration algorithms are designed and compared. Besides the exploration strategies, the paper reports a solution for quick convergence towards the actual stack position once detected by one member of the team. Both the navigation and localisation algorithms are fully distributed and based on the consensus theory. Simulations on realistic case studies are reported.

==> Introduction.old.tex <==
\section{Introduction and related works}
\label{sec:Introduction}

Unmanned Aerial Vehicles (UAVs), RPA (Remotely Pilot Aircraft) or
improperly dubbed {\em drones} are nowadays used for a large variety
of applications, such as structural
monitoring~\cite{yoon2018structural}, emergency scenarios like search
and rescue~\cite{SeminaraF17mesas,robocup16}, fault detection
occurring on airspeed sensors~\cite{Go13}, target tracking and
encircling~\cite{ow10,is13,MorelliVF17mesas}, reaching close to
commercial solutions in some cases~\cite{AmazonPJ, AWARD}. Thanks to
lighter structure and batteries with higher capacity, UAVs are
increasingly used in those situations where was difficult for human
being to carry out specific operations (e.g. in toxic or radioactive
environments). Moreover, UAVs usually lower the price of difficult
operations and, as in the situation described in this paper, they
generally behave better than other solutions or means of transport
used in the past years. The distinctive feature of this work relies on
the presence of multiple autonomous UAVs, and specifically
quadrotors~\cite{GPSaccuracy77, DronesTheory}, in order to speed up
the entire process of search and detection, and to precisely localise
the emission source.  In this respect, our solution can be roughly
divided into two steps: the first concerns the exploration strategies
towards the source detection, the second is more related to the
distributed localisation once the source has been detected.

% Exploration
The use of coordinated multiple agents is of course not novel in the
literature. In particular, it has been shown that the
information exchange between the agents of a team reduces to time to
accomplish a mission, which can be theoretically demonstrated, for
example applying the consensus theory~\cite{ren2005survey}.  In this
framework, UAV formation control using a completely distributed
approach among the controlled robots is a field already investigated
in the literature~\cite{zhu2015model}.  Solutions based on potential
fields has been recently proposed in~\cite{de2006formation}.

% Estimation
Once the stack has been detected, the UAVs have to estimate its
position.  The literature for target tracking is quite
rich~\cite{li2003survey,li2005survey, AndreettoPMPF18mdpi}, especially
when the target is not governed by a white noise but, instead, has a
strong correlation between the executed
manoeuvres~\cite{singer1970estimating}.  Assuming that the target is
not moving but it is standing in a fixed unknown location has also
been presented in the literature, for example
by~\cite{li2014cooperative, AndreettoPFM15} using distributed
consensus based known algorithms as~\cite{carli2008distributed,
  OlfatiDKF}.

The papers that are closer to the presented approach are
probably~\cite{Merino10,sinha2017cooperative,mamduh2018gas}.  The
approach proposed in~\cite{Merino10} is conceived for forest fire
monitoring, where a team of aircrafts detects and localises a fire as
well as participates in fire monitoring task with human
firefighters. The most important parameters in these cases are the
position of the fire and the height of flames in order to better
predict how the front evolves in time. This work is one of the few who
presents a solution with multiple UAVs exploiting the capability of
data fusion and image processing techniques. Moreover, the UAVs can
adapt their deployment to avoid the inconveniences of other
approaches, like the presence of smoke, or to cover the more
convenient places.

In~\cite{sinha2017cooperative}, a hierarchical cooperative control has
been put forward to solve the problem of locating source of an odor by
driving the agents using a consensus-based protocol. The proposed
control provides stability and ensures robustness even in the presence
of bounded disturbances and matched uncertainties. As for the gas
plume here considered, odour arrives in packets, leading to wide
fluctuations in measured concentrations due to wind direction, which
is considered measured in this approach.  The model of the team relies
on the graph theory, where agents are modelled as graph nodes while
the communication as a directed graph edge.

Gas source localisation is considered in~\cite{mamduh2018gas} using
the ``Grey Wolf Optimiser'', a recently developed algorithm inspired
by grey wolves (Canis lupus).  It consists in three stage procedure;
tracking the prey, encircling the prey, and attacking the prey.  This
algorithm works with a minimum of $4$ agents and increasing the agent
number beyond seven agents caused reduction in success rate
(percentage of success in gas source localisation, $72\%$ with $7$
agents) and increase the time to completion, due to increased
frequency of irrecoverable collisions between robots.

In this paper, three simple exploration algorithms for a team of UAVs
conceived for gas source localisation are proposed, which are dubbed
{\em scanning}, {\em Brownian} and {\em Random Walk}; the 3 algorithms
share the same logic: as long as one agent senses the gas with a
concentration greater than a certain threshold, it becomes the master
of the group and the source localisation phase starts.  In this latter
phase, the agents are controlled with a distributed algorithm that
dynamically allocates the master role and localises the source.  The
algorithms presented in this paper are able to converge on the maximum
concentration point, which is a property shared with the Particle
Swarm Operation~\cite{ferri2007explorative} and the Ant Colony
Optimisation~\cite{zou2009swarm} approaches. Nonetheless, the main
differences with the discussed literature is \dan{Input here} Finally,
for the estimation problem as well as for the exploration, we have
considered a limited sensing range for the UAVs, as
in~\cite{de2015board}.

The paper is organised as follows.  Section~\ref{sec:Models}
introduces the adopted models and presents the problem at hand. Then,
in Section~\ref{sec:Exploration} and in Section~\ref{sec:Localisation}
the algorithms used for the area exploration and the source
localisation are defined. Section~\ref{sec:Results} presents extensive
simulations analysing all the relevant features of the algorithms and
their comparison.  Finally, Section~\ref{sec:Conclusions} draws the
conclusions and discusses possible future developments.


==> introduction_old.tex <==
<<<<<<< HEAD
\section{Introduction and related works}
\label{sec:Introduction}

Unmanned Aerial Vehicles (UAVs), RPA (Remotely Pilot Aircraft) or
improperly dubbed {\em drones} are nowadays used for a large variety
of applications, such as structural
monitoring~\cite{yoon2018structural}, emergency scenarios like search
and rescue~\cite{SeminaraF17mesas,robocup16}, fault detection
occurring on airspeed sensors~\cite{Go13}, target tracking and
encircling~\cite{ow10,is13,MorelliVF17mesas}, reaching close to
commercial solutions in some cases~\cite{AmazonPJ, AWARD}. Thanks to
lighter structure and batteries with higher capacity, UAVs are
increasingly used in those situations where was difficult for human
being to carry out specific operations (e.g. in toxic or radioactive
environments). Moreover, UAVs usually lower the price of difficult
operations and, as in the situation described in this paper, they
generally behave better than other solutions or means of transport
used in the past years. The distinctive feature of this work relies on
the presence of multiple autonomous UAVs, and specifically
quadrotors~\cite{GPSaccuracy77, DronesTheory}, in order to speed up
the entire process of search and detection, and to precisely localise
the emission source.  In this respect, our solution can be roughly
divided into two steps: the first concerns the exploration strategies
towards the source detection, the second is more related to the
distributed localisation once the source has been detected.

% Exploration
The use of coordinated multiple agents is of course not novel in the
literature. In particular, it has been shown that the
information exchange between the agents of a team reduces to time to
accomplish a mission, which can be theoretically demonstrated, for
example applying the consensus theory~\cite{ren2005survey}.  In this
framework, UAV formation control using a completely distributed
approach among the controlled robots is a field already investigated
in the literature~\cite{zhu2015model}.  Solutions based on potential
fields has been recently proposed in~\cite{de2006formation}.

% Estimation
Once the stack has been detected, the UAVs have to estimate its
position.  The literature for target tracking is quite
rich~\cite{li2003survey,li2005survey, AndreettoPMPF18mdpi}, especially
when the target is not governed by a white noise but, instead, has a
strong correlation between the executed
manoeuvres~\cite{singer1970estimating}.  Assuming that the target is
not moving but it is standing in a fixed unknown location has also
been presented in the literature, for example
by~\cite{li2014cooperative, AndreettoPFM15} using distributed
consensus based known algorithms as~\cite{carli2008distributed,
  OlfatiDKF}.

The papers that are closer to the presented approach are
probably~\cite{Merino10,sinha2017cooperative,mamduh2018gas}.  The
approach proposed in~\cite{Merino10} is conceived for forest fire
monitoring, where a team of aircrafts detects and localises a fire as
well as participates in fire monitoring task with human
firefighters. The most important parameters in these cases are the
position of the fire and the height of flames in order to better
predict how the front evolves in time. This work is one of the few who
presents a solution with multiple UAVs exploiting the capability of
data fusion and image processing techniques. Moreover, the UAVs can
adapt their deployment to avoid the inconveniences of other
approaches, like the presence of smoke, or to cover the more
convenient places.

In~\cite{sinha2017cooperative}, a hierarchical cooperative control has
been put forward to solve the problem of locating source of an odor by
driving the agents using a consensus-based protocol. The proposed
control provides stability and ensures robustness even in the presence
of bounded disturbances and matched uncertainties. As for the gas
plume here considered, odour arrives in packets, leading to wide
fluctuations in measured concentrations due to wind direction, which
is considered measured in this approach.  The model of the team relies
on the graph theory, where agents are modelled as graph nodes while
the communication as a directed graph edge.

Gas source localisation is considered in~\cite{mamduh2018gas} using
the ``Grey Wolf Optimiser'', a recently developed algorithm inspired
by grey wolves (Canis lupus).  It consists in three stage procedure;
tracking the prey, encircling the prey, and attacking the prey.  This
algorithm works with a minimum of $4$ agents and increasing the agent
number beyond seven agents caused reduction in success rate
(percentage of success in gas source localisation, $72\%$ with $7$
agents) and increase the time to completion, due to increased
frequency of irrecoverable collisions between robots.

In this paper, three simple exploration algorithms for a team of UAVs
conceived for gas source localisation are proposed, which are dubbed
{\em scanning}, {\em Brownian} and {\em Random Walk}; the 3 algorithms
share the same logic: as long as one agent senses the gas with a
concentration greater than a certain threshold, it becomes the master
of the group and the source localisation phase starts.  In this latter
phase, the agents are controlled with a distributed algorithm that
dynamically allocates the master role and localises the source.  The
algorithms presented in this paper are able to converge on the maximum
concentration point, which is a property shared with the Particle
Swarm Operation~\cite{ferri2007explorative} and the Ant Colony
Optimisation~\cite{zou2009swarm} approaches. Nonetheless, the main
differences with the discussed literature is \dan{Input here} Finally,
for the estimation problem as well as for the exploration, we have
considered a limited sensing range for the UAVs, as
in~\cite{de2015board}.

The paper is organised as follows.  Section~\ref{sec:Models}
introduces the adopted models and presents the problem at hand. Then,
in Section~\ref{sec:Exploration} and in Section~\ref{sec:Localisation}
the algorithms used for the area exploration and the source
localisation are defined. Section~\ref{sec:Results} presents extensive
simulations analysing all the relevant features of the algorithms and
their comparison.  Finally, Section~\ref{sec:Conclusions} draws the
conclusions and discusses possible future developments.
=======
%<<<<<<< HEAD
%\section{Introduction and related works}
%\label{sec:Introduction}
%
%Unmanned Aerial Vehicles (UAVs), RPA (Remotely Pilot Aircraft) or
%improperly dubbed {\em drones} are nowadays used for a large variety
%of applications, such as structural
%monitoring~\cite{yoon2018structural}, emergency scenarios like search
%and rescue~\cite{SeminaraF17mesas,robocup16}, fault detection
%occurring on airspeed sensors~\cite{Go13}, target tracking and
%encircling~\cite{ow10,is13,MorelliVF17mesas}, reaching close to
%commercial solutions in some cases~\cite{AmazonPJ, AWARD}. Thanks to
%lighter structure and batteries with higher capacity, UAVs are
%increasingly used in those situations where was difficult for human
%being to carry out specific operations (e.g. in toxic or radioactive
%environments). Moreover, UAVs usually lower the price of difficult
%operations and, as in the situation described in this paper, they
%generally behave better than other solutions or means of transport
%used in the past years. The distinctive feature of this work relies on
%the presence of multiple autonomous UAVs, and specifically
%quadrotors~\cite{GPSaccuracy77, DronesTheory}, in order to speed up
%the entire process of search and detection, and to precisely localise
%the emission source.  In this respect, our solution can be roughly
%divided into two steps: the first concerns the exploration strategies
%towards the source detection, the second is more related to the
%distributed localisation once the source has been detected.
%
%% Exploration
%The use of coordinated multiple agents is of course not novel in the
%literature. In particular, it has been shown that the
%information exchange between the agents of a team reduces to time to
%accomplish a mission, which can be theoretically demonstrated, for
%example applying the consensus theory~\cite{ren2005survey}.  In this
%framework, UAV formation control using a completely distributed
%approach among the controlled robots is a field already investigated
%in the literature~\cite{zhu2015model}.  Solutions based on potential
%fields has been recently proposed in~\cite{de2006formation}.
%
%% Estimation
%Once the stack has been detected, the UAVs have to estimate its
%position.  The literature for target tracking is quite
%rich~\cite{li2003survey,li2005survey, AndreettoPMPF18mdpi}, especially
%when the target is not governed by a white noise but, instead, has a
%strong correlation between the executed
%manoeuvres~\cite{singer1970estimating}.  Assuming that the target is
%not moving but it is standing in a fixed unknown location has also
%been presented in the literature, for example
%by~\cite{li2014cooperative, AndreettoPFM15} using distributed
%consensus based known algorithms as~\cite{carli2008distributed,
%  OlfatiDKF}.
%
%The papers that are closer to the presented approach are
%probably~\cite{Merino10,sinha2017cooperative,mamduh2018gas}.  The
%approach proposed in~\cite{Merino10} is conceived for forest fire
%monitoring, where a team of aircrafts detects and localises a fire as
%well as participates in fire monitoring task with human
%firefighters. The most important parameters in these cases are the
%position of the fire and the height of flames in order to better
%predict how the front evolves in time. This work is one of the few who
%presents a solution with multiple UAVs exploiting the capability of
%data fusion and image processing techniques. Moreover, the UAVs can
%adapt their deployment to avoid the inconveniences of other
%approaches, like the presence of smoke, or to cover the more
%convenient places.
%
%In~\cite{sinha2017cooperative}, a hierarchical cooperative control has
%been put forward to solve the problem of locating source of an odor by
%driving the agents using a consensus-based protocol. The proposed
%control provides stability and ensures robustness even in the presence
%of bounded disturbances and matched uncertainties. As for the gas
%plume here considered, odour arrives in packets, leading to wide
%fluctuations in measured concentrations due to wind direction, which
%is considered measured in this approach.  The model of the team relies
%on the graph theory, where agents are modelled as graph nodes while
%the communication as a directed graph edge.
%
%Gas source localisation is considered in~\cite{mamduh2018gas} using
%the ``Grey Wolf Optimiser'', a recently developed algorithm inspired
%by grey wolves (Canis lupus).  It consists in three stage procedure;
%tracking the prey, encircling the prey, and attacking the prey.  This
%algorithm works with a minimum of $4$ agents and increasing the agent
%number beyond seven agents caused reduction in success rate
%(percentage of success in gas source localisation, $72\%$ with $7$
%agents) and increase the time to completion, due to increased
%frequency of irrecoverable collisions between robots.
%
%In this paper, three simple exploration algorithms for a team of UAVs
%conceived for gas source localisation are proposed, which are dubbed
%{\em scanning}, {\em Brownian} and {\em Random Walk}; the 3 algorithms
%share the same logic: as long as one agent senses the gas with a
%concentration greater than a certain threshold, it becomes the master
%of the group and the source localisation phase starts.  In this latter
%phase, the agents are controlled with a distributed algorithm that
%dynamically allocates the master role and localises the source.  The
%algorithms presented in this paper are able to converge on the maximum
%concentration point, which is a property shared with the Particle
%Swarm Operation~\cite{ferri2007explorative} and the Ant Colony
%Optimisation~\cite{zou2009swarm} approaches. Nonetheless, the main
%differences with the discussed literature is \dan{Input here} Finally,
%for the estimation problem as well as for the exploration, we have
%considered a limited sensing range for the UAVs, as
%in~\cite{de2015board}.
%
%The paper is organised as follows.  Section~\ref{sec:Models}
%introduces the adopted models and presents the problem at hand. Then,
%in Section~\ref{sec:Exploration} and in Section~\ref{sec:Localisation}
%the algorithms used for the area exploration and the source
%localisation are defined. Section~\ref{sec:Results} presents extensive
%simulations analysing all the relevant features of the algorithms and
%their comparison.  Finally, Section~\ref{sec:Conclusions} draws the
%conclusions and discusses possible future developments.
%=======
\section{Introduction and related works}
\label{sec:Introduction}

Unmanned Aerial Vehicles (UAVs), RPA (Remotely Pilot Aircraft) 
%or improperly dubbed {\em drones} 
are nowadays used for a large variety
of applications, such as structural
monitoring~\cite{yoon2018structural}, emergency scenarios like search
and rescue~\cite{SeminaraF17mesas}, 
%fault detection occurring on airspeed sensors~\cite{Go13}, 
target tracking and encircling~\cite{MorelliVF17mesas}, reaching close to
commercial solutions in some cases~\cite{AmazonPJ}, or environmental monitoring~\cite{Rossi2014,IEEESJ2014}.  
%, AWARD}.  %Thanks to
%lightweight structure and the high capacity batteries, UAVs are
%increasingly used in those situations where the direct human
%operations are difficult to carry out or unsafe (e.g. in toxic or
%radioactive environments, such as the nuclear disaster happened in
%Chernobyl in 1986 or the more recent Fukushima in 2011).

%Moreover, UAVs usually lower the price of difficult operations 
% and they generally fulfil the goal more effectively than other 
%means of transport used in the past years. 
%The contribution of this 
%work is based on multiple autonomous UAVs, and specifically, 
%quadrotors~\cite{GPSaccuracy77}, %DronesTheory}, 
%used to speed up the task of \textsl{seek-and-find}.

The goal of this work is to localise the emission source of the gas dispersion as fast as possible as proposed in~\cite{SAS2015}, using 
 multiple autonomous UAVs, and specifically, quadrotors~\cite{GPSaccuracy77}, to speed up the task of \textsl{seek-and-find}.
Our solution consists of two steps: the first concerns 
the exploration strategies towards the gas source detection, 
the second focuses on the distributed localisation once 
the source has been detected. 

%Moreover, UAVs usually lower the price of difficult
%operations and, as in the situation described in this paper, they
%generally behave better than other solutions or means of transport
%used in the past years. The distinctive feature of this work relies on
%the presence of multiple autonomous UAVs, and specifically
%quadrotors~\cite{GPSaccuracy77, DronesTheory}, in order to speed up
%the entire process of search and detection, and to precisely localise
%the emission source.  In this respect, our solution can be roughly
%divided into two steps: the first concerns the exploration strategies
%towards the source detection, the second is more related to the
%distributed localisation once the source has been detected.

% Exploration
The use of coordinated multiple agents is of course not novel in the
literature. In particular, it has been shown that the
information exchange between the agents of a team reduces to time to
accomplish a mission, which can be theoretically demonstrated, for
example applying the consensus theory~\cite{ren2005survey}.  In this
framework, UAV formation control using a completely distributed
approach among the controlled robots is a field already investigated
in the literature~\cite{zhu2015model}.  
%Solutions based on potential fields have been recently proposed in~\cite{de2006formation}.

% Estimation
Once the stack has been detected, the UAVs have to estimate its
position.  The literature for target tracking is quite
rich~\cite{li2005survey, AndreettoPMPF18mdpi}, especially
when the target is not governed by a white noise but, instead, has a
strong correlation between the executed
manoeuvres~\cite{singer1970estimating}.  Assuming that the target is
not moving but it is standing in a fixed unknown location has also
been presented in the literature, for example
by~\cite{li2014cooperative, AndreettoPFM15} using distributed
consensus-based known algorithms. % as~\cite{carli2008distributed,OlfatiDKF}.

% The papers that are closer to the presented approach are
% probably~\cite{Merino10,sinha2017cooperative,mamduh2018gas}.  The
% approach proposed in~\cite{Merino10} is conceived for forest fire
% monitoring, where a team of aircrafts detects and localises a fire as
% well as participates in fire monitoring task with human
% firefighters. The most important parameters in these cases are the
% position of the fire and the height of the flames to better
% predict how the front evolves in time. 
% 
%This work is one of the few who
%presents a solution with multiple UAVs exploiting the capability of
%data fusion and image processing techniques. Moreover, the UAVs can
%adapt their deployment to avoid the inconveniences of other
%approaches, like the presence of smoke, or to cover the more
%convenient places.

% In~\cite{sinha2017cooperative}, a hierarchical cooperative control has
% been used to solve the problem of locating source of an odour by
% driving the agents using a consensus-based protocol. The proposed
% control provides stability and ensures robustness even in the presence
% of bounded disturbances and matched uncertainties. 
% 
%As for the gas
%plume here considered, odour arrives in packets, leading to wide
%fluctuations in measured concentrations due to wind direction, which
%is considered measured in this approach.  The model of the team relies
%on the graph theory, where agents are modelled as graph nodes while
%the communication as a directed graph edge.

Gas source localisation is considered in~\cite{mamduh2018gas} using
the ``Grey Wolf Optimiser'', a recently developed algorithm inspired
by grey wolves (Canis lupus).  It consists of three-stage procedure:
tracking the prey, encircling the prey, and attacking the prey.  This
algorithm works with a minimum of $4$ agents and, increasing the agent
number beyond seven, caused the reduction in success rate (percentage
of success in gas source localisation, $72\%$ with $7$ agents) and
increase the time to completion, due to increased frequency of
irrecoverable collisions between robots.

In this paper, three exploration algorithms for swarms of UAVs
conceived for gas source localisation are proposed and are based on i)
{\em coordinated scanning}, ii) {\em Random walk} and iii) {\em
  Brownian motion}.  All share the same method: as long as one agent
senses the gas with a concentration greater than a certain threshold,
it becomes the master of the group and the source localisation phase
starts.
%
%In this paper, three simple exploration algorithms for a team of UAVs
%conceived for gas source localisation are proposed, which are dubbed
%{\em scanning}, {\em Brownian} and {\em Random Walk}; the 3 algorithms
%share the same logic: as long as one agent senses the gas with a
%concentration greater than a certain threshold, it becomes the master
%of the group and the source localisation phase starts.  
In this latter phase, the agents are controlled with a distributed
algorithm that dynamically allocates the master role and localises the
source.  The algorithms presented in this paper converge on the
maximum concentration point, which is a property shared with the
Particle Swarm Operation~\cite{ferri2007explorative} and the Ant
Colony Optimisation~\cite{zou2009swarm} approaches.  Nonetheless,
there are some differences with respect to the discussed literature,
the most relevant being the approach adopted to find the source. In
fact, in the Grey Wolf Optimiser, agents start in a zone where the
concentration of the gas is above a minimum sensing threshold, and
this data is necessary to reach the source; in our case, instead, UAVs
can start in any part of the environment.  Moreover, we can
statistically prove through extensive simulations that our algorithms
can operate also with 2 drones instead of a minimum of 4 and that the
rate of success under the presented assumptions is 100\%.
%
%Nonetheless, the main
%differences with the discussed literature is \dan{Input here} 
%
Finally, for the estimation problem as well as for the exploration, we
have considered a limited sensing range for the UAVs, as
in~\cite{de2015board}.

The paper is organised as follows.  Section~\ref{sec:Models}
introduces the adopted models and presents the problem at hand. Then,
in Section~\ref{sec:Exploration} and in Section~\ref{sec:Localisation}
the algorithms used for the area exploration and the source
localisation are defined. Section~\ref{sec:Results} presents extensive
simulations analysing all the relevant features of the algorithms and
their comparison.  Finally, Section~\ref{sec:Conclusions} draws the
conclusions and discusses possible future developments.
%>>>>>>> 2282541dd0a8fc19b27c0ab32df818522cdca2fd
%>>>>>>> camera_ready

